From Continuity to Editability: Inverting GANs with Consecutive Images

Existing GAN inversion methods are stuck in a paradox that the inverted codes can either achieve high-fidelity reconstruction, or retain the editing capability. Having only one of them clearly cannot realize real image editing. In this paper, we resolve this paradox by introducing consecutive images (\eg, video frames or the same person with different poses) into the inversion process. The rationale behind our solution is that the continuity of consecutive images leads to inherent editable directions. This inborn property is used for two unique purposes: 1) regularizing the joint inversion process, such that each of the inverted code is semantically accessible from one of the other and fastened in a editable domain; 2) enforcing inter-image coherence, such that the fidelity of each inverted code can be maximized with the complement of other images. Extensive experiments demonstrate that our alternative significantly outperforms state-of-the-art methods in terms of reconstruction fidelity and editability on both the real image dataset and synthesis dataset. Furthermore, our method provides the first support of video-based GAN inversion, and an interesting application of unsupervised semantic transfer from consecutive images. Source code can be found at: \url{https://github.com/cnnlstm/InvertingGANs_with_ConsecutiveImgs}.

==> compare_table.tex <==

\begin{table}[t]
   \caption{Optimization spaces and tasks on different inversion methods}
       \vspace{-0.6cm}
       \begin{center}
       \setlength{\tabcolsep}{0.1cm}{
       \begin{tabular}{c|c|c|c|c|c|c}
           \hline
           {Methods}        &{I2S}  &{I2S++}    &{pSp}   &{InD}   & Ours     & Ours++\\
           \hline
           $\mathcal{W+}$ &$\checkmark$ &$\checkmark$ &$\checkmark$ &$\checkmark$ &$\checkmark$ &$\checkmark$  \\
           $\mathcal{N}$  &$\times$     &$\checkmark$ &$\times$     &$\times$     &$\times$     &$\checkmark$ \\
           \hline
           Reconstruction &$\checkmark$   &$\checkmark$ &$\checkmark$    &$\checkmark$ &$\checkmark$    &$\checkmark$ \\
           Editing          &$\checkmark$   &$\times$    &$\checkmark$     &$\checkmark$ &$\checkmark$     &$\times$ \\
           \hline
       \end{tabular}
       }
      \end{center}
      \label{table:competitors}
      \vspace{-6mm}
\end{table}


==> teaser.tex <==
%!TeX root = egpaper_for_review.tex


\begin{figure}[t]
   \centering
    \hspace{-5mm}
    \vspace{5mm}
    \subfloat[Input]{
    \begin{minipage}{0.195\linewidth}
     \includegraphics[width=\linewidth]{figure/teaser/truth/tesla_3}
     \includegraphics[width=\linewidth]{figure/teaser/truth/tesla_3}
     \includegraphics[width=\linewidth]{figure/teaser/truth/tesla_3}
     \end{minipage}
     }
   \hspace{-2.2mm}
   \subfloat[Ours]{
     \begin{minipage}{0.195\linewidth}
     \includegraphics[width=\linewidth]{figure/teaser/ours/tesla_3}
     \includegraphics[width=\linewidth]{figure/teaser/ours/tesla_3_pose_+1}
     \includegraphics[width=\linewidth]{figure/teaser/ours/tesla_3_smile_+1}
     % \includegraphics[width=\linewidth]{figure/teaser/ours/000065_2_age_+1}
     \end{minipage}
     }
   \hspace{-2.8mm}
   \subfloat[I2S~\cite{abdal2019image2stylegan}]{
     \begin{minipage}{0.195\linewidth}
     \includegraphics[width=\linewidth]{figure/teaser/i2s/tesla_3}
     \includegraphics[width=\linewidth]{figure/teaser/i2s/tesla_3_pose_+1}
     \includegraphics[width=\linewidth]{figure/teaser/i2s/tesla_3_smile_+1}
     \end{minipage}
     }
   \hspace{-2.8mm}
    \subfloat[Ind~\cite{zhu2020domain}]{
     \begin{minipage}{0.195\linewidth}
     \includegraphics[width=\linewidth]{figure/teaser/ind/tesla_3}
     \includegraphics[width=\linewidth]{figure/teaser/ind/tesla_3_pose_+1}
     \includegraphics[width=\linewidth]{figure/teaser/ind/tesla_3_smile_+1}
     \end{minipage}
     }
   \hspace{-2.8mm}
    \subfloat[pSp~\cite{richardson2020encoding}]{
     \begin{minipage}{0.195\linewidth}
     \includegraphics[width=\linewidth]{figure/teaser/psp/tesla_3}
     \includegraphics[width=\linewidth]{figure/teaser/psp/tesla_3_pose_+1}
     \includegraphics[width=\linewidth]{figure/teaser/psp/tesla_3_smile_+1}
     \end{minipage}
     }
   \hspace{-1mm}
   \rotatebox[origin=c]{270}{\hspace{-2mm}Inversion\hspace{7mm}Pose\hspace{7mm}Smile}
\hspace{-10mm}
\caption{GAN inversion and semantic editing on the real image. Our proposed method can invert a more realistic image and the inverted latent code is more favorable for semantics editing.}
\label{fig:semantic_teaser}\vspace{-3mm}
\end{figure}

